Planet Hunters TESS II: Findings from the first two years of TESS

We present the results from the first two years of the Planet Hunters TESS citizen science project, which identifies planet candidates in the TESS data by engaging members of the general public. Over 22,000 citizen scientists from around the world visually inspected the first 26 Sectors of TESS data in order to help identify transit-like signals. We use a clustering algorithm to combine these classifications into a ranked list of events for each sector, the top 500 of which are then visually vetted by the science team. We assess the detection efficiency of this methodology by comparing our results to the list of TESS Objects of Interest (TOIs) and show that we recover 85 % of the TOIs with radii greater than 4 Earth radii and 51 % of those with radii between 3 and 4 Earth radii. Additionally, we present our 90 most promising planet candidates that had not previously been identified by other teams, 73 of which exhibit only a single transit event in the TESS light curve, and outline our efforts to follow these candidates up using ground-based observatories. Finally, we present noteworthy stellar systems that were identified through the Planet Hunters TESS project.

==> PHT Method Paper -arxiv/targets.tex <==
\appendix
\section{Planet candidate descriptions}
\label{appendixA}

A short outline all of the planet candidates, and any conclusions drawn from follow-up observations (where available). A more in depth description of the ground-based data will be presented in a follow-up paper. Unless stated otherwise, these candidates are not TOIs at the time of writing. Candidates for which we have no additional information to complement the results presented in Table~\ref{tab:PHT-caniddates} are not discussed further here.

\subsection{Single-transit planet candidates}

%\textbf{TIC 101641905.} Single transit event identified in Sector 22.

\textbf{TIC 103633672.} Single transit event identified in Sector 20. The single LCO/NRES spectra shows no sign of this being a double lined spectroscopic binary.  We caution that there is a star on the same pixels, which is 0.1 mag brighter. We are unable to rule this star out as the cause for the transit-like signal.

\textbf{TIC 110996418.} Single transit event identified in Sector 10. We caution that there is a star on the same \tess\ pixel, which is 2.4 magnitudes fainter than the target.

\textbf{TIC 128703021.} Single transit event identified in Sector 11. With a stellar radius of 1.6 $R_{\odot}$ and a T$_{eff}$ of 6281 this host star is likely in the subgiant phase of its evolution. The 43 spectra obtained with MINERVA australis and the two obtained with LCO/NRES are consistent with a planetary nature. Gemini speckle interferometry shows no nearby companion stars.

%\textbf{TIC 138126035} Single transit event identified in Sector 23.

\textbf{TIC 142087638.} Single transit event identified in Sector 7. The best fit \pyaneti\ model of the transit suggests an orbital period of only 3.14 d. As there are no additional transits seen in the light curve, this period is clearly not possible. We caution that the transit is most likely caused by a grazing object, and is therefore likely to be caused by a stellar companion. However, without further data we are unable to rule this candidate out as being planetary in nature.

\textbf{TIC 159159904.} Single transit event identified in Sector 22. The initial two observations obtained using LCO/NRES show no sign of the candidate being a double lined spectroscopic binary.

%\textbf{TIC 162631539} Single transit event identified in Sector 24.

\textbf{TIC 166184426.} Single transit event identified in Sector 11. Since the PHT discovery this cTOI has been become the priority 1 (1=highest, 5=lowest) target TOI  1955.01.


\textbf{TIC 172370679.} Single transit event identified in Sector 15. \textcolor{black}{This candidate was independently discovered and verified using a BLS algorithm used to search for transiting planets around M-dwarfs. The candidate is now the confirmed planet TOI 1899 b \citep{canas2020}.} 

\textbf{TIC 174302697.} Single transit event identified in Sectors 16. With a stellar radius of 1.6 $R_{\odot}$ and a T$_{eff}$ of 6750 this host star is likely in the subgiant phase of its evolution. \textcolor{black}{This candidate was initially flagged as a TCE and but was erroneously discounted due to the pipeline mistaking the data glitch at the time of a momentum dump as a secondary eclipse.} Since the PHT discovery this cTOI has become the priority 3 target TOI 1896.01. 

\textbf{TIC 192415680.} Single transit event identified in Sector 18. The two epochs of RV measurement obtained with OHP/SOPHIE are consistent with a planetary scenario.

\textbf{TIC 192790476.} Single transit event identified in Sector 5. This target has been identified to be a wide binary with am angular separation of 72.40 arcseconds \citep{andrews2017wideBinary} and a period of 162705 years \citep{benavides2010new}. The star exhibits large scale variability on the order of around 10 d. The signal is consistent with that of spot modulations, which would suggest that this is a slowly rotating star.

%\textbf{TIC 206361691} CHIRON spectra revealed that this is a spectroscopic binary.

%\textbf{TIC 207501148} Single transit event identified in Sector 25.

\textbf{TIC 219466784.} Single transit event identified in Sector 22. We caution that there is a nearby companion located within the same \tess\ pixel at an angular separation of 16.3 with a Vmag of 16.3". Since the PHT discovery this cTOI has become the priority 2 target TOI  2007.01.


%\textcolor{black}{\textbf{TIC 224307602. KILLED} Single transit event identified in Sector 24. With a stellar radius of 2.0 $R_{\odot}$ and a T$_{eff}$ of 6658 K this host star is likely in the subgiant phase of its evolution. We note that there is a second star on the same \tess\ pixel as TIC 224307602, however, as this star is 7.6 magnitude fainter than the target, we can the companion out as being the source of the transit like signal.}

\textbf{TIC 229055790.} Single transit event identified in Sector 21. We note that the midpoint of the transit-like events coincides with a \tess\ momentum dump, however, we believe the shape to be convincing enough to warrant further investigation. The two LCO/NRES spectra show no sign of this being a spectroscopic binary.

\textbf{TIC 229608594.} Single transit event identified in Sector 24. Since the PHT discovery this cTOI has become the priority 3 target TOI 2298.01.



\textbf{TIC 233194447.} Single transit event identified in Sector 14. The transit-like event is shallow and asymmetric and we cannot definitively rule out systematics as the cause for the event without additional data. The initial two LCO/NRES spectra show no sign of this target being a spectroscopic binary.

\textbf{TIC 237201858.} Single transit event identified in Sector 18. The single LCO/NRES spectra shows no sign of this being a double lined spectroscopic binary.

\textbf{TIC 243187830.} Single transit event identified in Sector 18. There are no nearby bright stars. \textcolor{black}{This light curve was initially flagged as a TCE, however, the flagged events corresponded to stellar variability and not the same event identified by PHT.} The single LCO/NRES spectrum shows no sign of this being a double lined spectroscopic binary. Since the PHT discovery this cTOI has become the priority 3 target TOI 2009.01.

\textbf{TIC 243417115.} Single transit event identified in Sector 11. We note that the best fit \pyaneti\ model of the transit suggests an orbital period of only 1.81 d. As there are no additional transits seen in the light curve, this period is clearly not possible. We caution that the transit is most likely caused by a grazing object, and is therefore likely to be caused by a stellar companion. However, without further follow-up data we are unable to rule this candidate out as being planetary in nature.

%\textbf{TIC 256429408} Single transit event identified in Sector 24.

\textbf{TIC 264544388.} Single transit event identified in Sector 19. The single LCO/NRES spectra shows no sign of this being a double lined spectroscopic binary. Apart from the single transit event, the light curve shows no obvious signals. A periodogram of the light curve, however, reveals a series of five significant peaks, nearly equidistantly spaced by $\sim1.03$~d$^{-1}$. Additionally, a rotationally split quintuplet is visible at 7.34~d$^{-1}$, with a splitting of $\sim0.12$~d$^{-1}$, suggesting an $\ell=2$ p-mode pulsation. The Maelstrom code \citep{hey2020maelstrom} revealed pulsation timing variations which are consistent with a long period planet. \textcolor{black}{The short period signal, which was also identified by the periodogram, was flagged as a TCE, however, the single-transit event was not flagged as a TCE.} Since the PHT discovery this cTOI has become the priority 3 target TOI 1893.01.

\textbf{TIC 264766922.} Single transit event identified in Sector 8. With a stellar radius of 1.7 $R_{\odot}$ and a T$_{eff}$ of 6913 K this host star is likely entering the subgiant phase of its evolution. The V-shape of this transit and the resultant high impact parameter suggests that the object is grazing. We can therefore not rule out that this candidate it a grazing eclipsing binary.  There are clear p-mode pulsations at frequencies of 9.01 and 11.47 cycles per day, as well as possible g-mode pulsations. \textcolor{black}{A very short period signal within this light curve was flagged as a TCE, however, the single transit event was ignored by the pipeline.}

\textbf{TIC 26547036.} Single transit event identified in Sector 14. The four LCO/NRES observations are consistent with the target being a planetary body and show no sign of the signal being caused by a spectroscopic binary. We caution that there is a star on the same \tess\ pixel, however, this star is 8.2 magnitudes fainter than the target, and therefore unable to be responsible for the transit event seen in the light curve. Gemini speckle interferometry reveal no additional nearby companion stars. \textcolor{black}{This candidate was initially flagged as a TCE, however, in addition to the single transit event the pipeline identified further periodic signals that correspond to times of momentum dumps. Due to this, the candidate was never promoted to TOI status.}

%\textbf{TIC 270371513} MINERVA australis spectra revealed that this is a spectroscopic binary.

\textbf{TIC 278990954.} Single transit event identified in Sector 12. With a stellar radius of 2.6 $R_{\odot}$ and a T$_{eff}$ of 5761 K this host star is likely in the subgiant phase of its evolution. We note that there are two additional stars on the same pixel as TIC 278990954. These two stars are 2.7 and 3.7 magnitudes fainter in the v-band than the target and can't be ruled out as the cause for the transit-like event without additional follow-up data.

\textbf{TIC 280865159.} Single transit event identified in Sector 16. Gemini speckle interferometry revealed any nearby companion stars. Since the PHT discovery this cTOI has become the priority 3 target TOI 1894.01.

\textbf{TIC 284361752.} Single transit event identified in Sector 26. Since the PHT discovery this cTOI has become the priority 2 target TOI 2294.01.


%\textbf{TIC 293649602} Single transit event identified in Sector 7.
\textbf{TIC 296737508.} Single transit event identified in Sector 8. The single LCO/NRES and the single MINERVA australis spectra show no sign of this being a spectroscopic binary. The Sinistro snapshot image revealed no additional nearby companions.

\textbf{TIC 298663873.} Single transit event identified in Sector 19. The two LCO/NRES spectra show no sign of this being a spectroscopic binary. With a stellar radius of 1.6 $R_{\odot}$ and a T$_{eff}$ of 6750 this host star is likely in the subgiant phase of its evolution. Gemini speckle images obtained by other teams show no signs of there being nearby companion stars. Since the PHT discovery this cTOI has become the priority 3 target TOI 2180.01.


\textbf{TIC 303050301.} Single transit event identified in Sector 2. The variability of the light curve is consistent with spot modulation. A single LCO/NRES spectrum shows no signs of this being a double lined spectroscopic binary.

\textbf{TIC 303317324.} Single transit event identified in Sector 2. We note that a second transit was later seen in Sector 29, however, as this work only covers sectors 1-26 of the primary \tess\ mission, this candidates is considered a single-transit event in this work. 

%\textbf{TIC 303586471} MINERVA australis spectra revealed that this is a spectroscopic binary.

\textbf{TIC 304142124.} Single transit event identified in Sector 10.\textcolor{black}{This target was independently identified as part of the Planet Finder Spectrograph, which uses precision RVs \citep{diaz2020}. This candidate is know the confirmed planet HD 95338 b.}


%\textbf{TIC 304339227} Single transit event identified in Sector 13.

%\textbf{TIC 307958020} Single transit event identified in Sector 20.

%\textbf{TIC 308301091} Single transit event identified in Sector 26. 

%\textbf{TIC 313006381} Single transit event identified in Sector 20. 

%\textbf{TIC 323295479} Single transit event identified in Sector 11.

\textbf{TIC 331644554.} Single transit event identified in Sector 16. There is a clear mono-periodic signal in the periodogram at around 11.2 cycles per day, which is consistent with p-mode pulsation.

\textbf{TIC 332657786.} Single transit event identified in Sector 8. We caution that there is a star on the adjacent \tess\ pixel that is brighter in the V-band by 2.4 magnitudes. At this point we are unable to rule out this star as the cause of the transit-like signal. 

%\textbf{TIC 336075472} Single transit event identified in Sector 26. 

\textbf{TIC 356700488.} Single transit event identified in Sector 16. There is a clear mono-periodic signal in the periodogram at around 1.2 cycles per day, which is consistent with either spot modulation or g-mode pulsation. However, there is no clear signal visible in the light curve that would allow us to differentiate between these two scenarios based on the morphology of the variation. Since the PHT discovery this cTOI has become the priority 3 target TOI 2098.01.

\textbf{TIC 356710041.} Single transit event identified in Sector 23. With a stellar radius of 2.8 $R_{\odot}$ and a T$_{eff}$ of 5701 K this host star is likely in the subgiant phase of its evolution. \textcolor{black}{This candidate was initially flagged as a TCE, however, in addition to the single transit event, the pipeline identified a further event that corresponds to the time of a momentum dump. Due to this the candidate failed the `odd-even test' and was initially discarded as a TOI.} Since the PHT discovery this cTOI has become the priority 3 target TOI 2065.01

\textbf{TIC 369532319.} Single transit event identified in Sector 16. Gemini speckle interferometry revealed no nearby companion stars.

%\textbf{TIC 369779127} Single transit event identified in Sector 12.

\textbf{TIC 384159646.} Single transit event identified in Sector 12. The eight LCO/NRES and six MINERVA australis spectra are consistent with this candidate being a planet. Both the SBIG snapshot and the Gemini speckle interferometry observations revealed no companion stars. Since the PHT discovery this cTOI has become the priority 3 target TOI 1895.01.


%\textbf{TIC 388134787} Single transit event identified in Sector 18.

%\textbf{TIC 404518509.} Single transit event identified in Sector 4.

\textbf{TIC 418255064.} Single transit event identified in Sector 12. The Gemini speckle image shows no sign of nearby companions.

%\textbf{TIC 420645189} MINERVA australis spectra revealed that this is a spectroscopic binary.

\textbf{TIC 422914082.} Single transit event identified in Sector 4. Single Sinistro snapshot image reveals no additional nearby stars.

\textbf{TIC 427344083.} Single transit event identified in Sector 24. We note that there is a star on the adjacent \tess\ pixel to the target, which is 3.5 magnitude fainter in the V-band than the target star. We also caution that the V-shape of the transit and the high impact parameter suggest that this is a grazing transit. However, without additional follow-up observations we are unable to rule this candidate out as a planet.


\textbf{TIC 436873727.} Single transit event identified in Sector 18. The host star shows strong variability on the order of one day, which is consistent with spot modulations or g-mode pulsations. The periodogram reveals multi-periodic behaviour in the low frequency range consistent with g-mode pulsations. 

\textbf{TIC 452920657.} Single transit event identified in Sector 17. The V-shape of this transit suggests that the object is grazing and future follow-up observations may reveal this to be an EB. \textcolor{black}{This candidate was initially flagged as a TCE, however, in addition to the single transit event, the pipeline identified a further two event that corresponds to likely stellar variability. Due to this the candidate failed the `odd-even test' and was initially discarded as a TOI.}

\textbf{TIC 455737331.} Single transit event identified in Sector 17. We note that there is a star on the same \tess\ pixel as the target, which is 4.5 magnitudes fainter in the V-band. Neither the SBIG snapshot nor the Gemini speckle interferometry revealed any further nearby companion stars.

\textbf{TIC 456909420.} Single transit event identified in Sector 17. We caution that the V-shape of the transit and the high impact parameter suggest that this is a grazing transit. However, without additional follow-up observations we are unable to rule this candidate out as a planet.

%\textbf{TIC 458451774} Single transit event identified in Sector 22.


%\textbf{TIC 53309262.} Single transit event identified in Sector 20.

\textbf{TIC 53843023.} Single transit event identified in Sector 1. We caution that the high impact parameter returned by the best fit \pyaneti\ model suggests that the transit event is caused by a grazing body. However, at this point we are unable to rule this candidate out as being planetary in nature.

\textbf{TIC 63698669.} Single transit event identified in Sector 2. The SBIG snapshot image revealed no nearby companions. \textcolor{black}{This candidate was initially identified as a TCE, however, in addition to the single transit event, the pipeline identified a further 3 events the light curve. Due to these, additional events, which correspond to stellar variability, the candidate was not initially promoted to TOI status.} However, since the PHT discovery this cTOI has become TOI 1892.01.

\textbf{TIC 70887357.} Single transit event identified in Sector 5. With a stellar radius of 2.1 $R_{\odot}$ and a T$_{eff}$ of 5463 K this host star is likely in the subgiant phase of its evolution. \textcolor{black}{This candidate was initially flagged as a TCE, however, in addition to the single transit-event the pipeline identified a further signal, and thus failed the `odd-even' transit test.} However, since the PHT discovery this cTOI has become the priority 3 target TOI 2008.01.

%\textbf{TIC 7422496} MINERVA australis spectra revealed that this is a spectroscopic binary.

%\textbf{TIC 88840705} Single transit event identified in Sector 26.

\textbf{TIC 91987762.} Single transit event identified in Sector 21. \textcolor{black}{This candidate was initially flagged as a TCE, however, in addition to the single transit-event the pipeline identified a further signal, and thus failed the `odd-even' transit test.} Since the PHT discovery this cTOI has become the priority 3 target TOI 1898.01.

%\textbf{TIC 95768667} Single transit event identified in Sector 22.


\subsection{Multi-transit and multi-planet candidates}


\textbf{TIC 160039081.} Multi-transit candidate with a period of 30.2 d. Single LCO/NRES spectra shows no sign of this being a double lined spectroscopic binary and a snapshot image using SBIG shows no nearby companions. The Gemini speckle images also show no additional nearby companions. Since the PHT discovery this cTOI has  become the priority 1 target TOI 2082.01.

\textbf{TIC 167661160.} Multi-transit candidate with a period of 36.8 d. The nine LCO/NRES and four MINERVA australis spectra have revealed this to be a long period eclipsing binary.

\textbf{TIC 179582003.} Multi-transit candidate with a period of 104.6 d. There is a clear mono-periodic signal in the periodogram at around 0.59 cycles per day, which is consistent with either spot modulation or g-mode pulsation. We caution that this candidate is located in a crowded field. With a stellar radius of 2.0 $R_{\odot}$ and a T$_{eff}$ of 6115 K this host star is likely in the subgiant phase of its evolution.

\textbf{TIC 219501568.} Multi-transit candidate with a period of 16.6 d. With a stellar radius of 1.7 $R_{\odot}$ and a T$_{eff}$ of 6690 K this host star is likely entering the subgiant phase of its evolution. \textcolor{black}{This candidate was identified as a TCE, however, it was not initially promoted to TOI status as the signal was thought to be off-target by the automated pipeline.} However, since the PHT discovery this cTOI has become the priority 3 target TOI 2259.01

\textbf{TIC 229742722.} Multi-transit candidate with a period of 63.48 d. Eight LCO/NRES and four OHP/SOPHIE observations are consistent with this candidate being a planet. Gemini speckle interferometry reveals no nearby companion stars. \textcolor{black}{This candidate was flagged as a TCE in sector 20, where it only exhibits a single transit event. An additional event was identified at the time of a momentum dump, and as such it failed the `odd-even' test and was not initially promoted to TOI status.} However, since the PHT discovery this cTOI has become the priority 3 target TOI 1895.01.

\textbf{TIC 235943205.} Multi-transit candidate with a period of 121.3 d. The LCO/NRES and OHP/SOPHIE observations remain consistent with a planetary nature of the signal. Since the PHT discovery this cTOI has become the priority 3 target TOI 2264.01.


\textbf{TIC 267542728.} Multi-transit event with period of 39.7 d. Observations obtained with Keck showed that the RV shifts are not consistent with a planetary body and are most likely due to an M-dwarf companion.

\textbf{TIC 274599700.} Multi-transit candidate with a period of 33.0 d. One of the two transit-like even is only half visible, with the other half of the event falling in a \tess\ data gap.

%\textbf{TIC 288240183} Multi-transit candidate with a period of 119.1 d.

%\textbf{TIC 29169215} Multi-transit candidate with a period of 14.9 d.

\textbf{TIC 328933398.} Multi-planet candidates. The 2-minute cadence light curve shows two single transit events of different depths across two \tess\ sectors, both of which are consistent with an independent planetary body. In addition to the short cadence data, this target was observed in an additional three sectors as part of the 30-minute cadence full frame images. These showed additional transit events for one of the planet candidates, with a period of 24.9 d. \textcolor{black}{This light curve was initially flagged as containing a TCE event, however, the two 2-minute cadence single transit events were thought to belong to the same transiting planet. The TCE was initially discarded as the pipeline identified the events to be off-target.} However, since the PHT discovery these two cTOIs has become the priority 3 and 1 targets, TOI 1873.01 and TOI 1873.01, respectively.

\textbf{TIC 349488688.} Multi-planet candidate, with one single transit event and one multi-transit candidate with a period of 11 d. Two LCO/NRES and two OHP/SOPHIE spectra, along with ongoing HARPS North are consistent with both of these candidates being planetary in nature. \textcolor{black}{The single transit event was initially identified as a TCE, however, in addition to the event it identified two other signals at the time of momentum dumps, and was therefore initially discarded by the pipeline as it failed the `odd-even' transit test.} However, since the PHT discovery the two-transit event has become the 1 targets, TOI 2319.01 (Eisner et al. in prep).

\textbf{TIC 385557214.} Multi-transit candidate with a period of 5.6 d. The prominent stellar variation seen in the light curve is likely due to spots or pulsation The high impact parameter returned by the best fit \pyaneti\ modelling suggests that the transit is likely caused by a grazing object. Without further observations, however, we are unable to rule this candidate out as being planetary in nature. \textcolor{black}{This candidate was flagged as a TCE but was not promoted to TOI status due to the other nearby stars.}

\textbf{TIC 408636441.} Multi-transit candidate with a period of 18.8 or 37.7 d. Due to \tess\ data gaps, half of the period stated in Table~\ref{tab:PHT-caniddates} is likely. The SBIG snapshot and Gemini speckle images show no signs of companion stars. \textcolor{black}{This candidate was flagged as a TCE in sector 24, where it only exhibits a single transit event. An additional event was identified at the time of a momentum dump, and as such it failed the `odd-even' test and was not initially promoted to TOI status.} However, since the PHT discovery this cTOI has become the priority 3 target TOI 1759.01.

\textbf{TIC 441642457.} Multi-transit candidate with a period of 79.8 d. \textcolor{black}{This candidate was flagged as a TCE in sector 14, where it only exhibits a single transit event. An additional event was identified at the time of a momentum dump, and as such it failed the `odd-even' test and was not initially promoted to TOI status.} Since the PHT discovery this cTOI has become the priority 2 target TOI 2073.01.

\textbf{TIC 441765914.} Multi-transit candidate with a period of 161.6 d.  Since the PHT discovery this cTOI has become the priority 1 target TOI 2088.01.

\textbf{TIC 48018596.} Multi-transit candidate with a period of 100.1 days (or a multiple thereof). The single LCO/NRES spectrum shows no sign of this target being a double lined spectroscopic binary. Gemini speckle interferometry revealed no nearby companion stars.  \textcolor{black}{This candidate was initially flagged as a TCE, however, in addition to the transit-events, the pipeline classified, what we consider stellar variability as an additional event. As such it failed the `odd-even' transit test and wasn't promoted to TOI status.} However, since the PHT discovery this cTOI has become the priority 3 target TOI 2295.01.

\textbf{TIC 55525572.} Multi-transit candidate with a period of 83.9 d. Since the PHT discovery this cTOI has become the confirmed planet TOI 813 \citep{2020eisner}.

\textbf{TIC 82452140.} Multi-transit candidate with a period of 21.1 d. Since the PHT discovery this cTOI has become the priority 2 target TOI 2289.01.


